DeltaGAN: Towards Diverse Few-shot Image Generation with Sample-Specific Delta

Learning to generate new images for a novel category based on only a few images, named as few-shot image generation, has attracted increasing research interest. Several state-of-the-art works have yielded impressive results, but the diversity is still limited. In this work, we propose a novel Delta Generative Adversarial Network (DeltaGAN), which consists of a reconstruction subnetwork and a generation subnetwork. The reconstruction subnetwork captures intra-category transformation, i.e., "delta", between same-category pairs. The generation subnetwork generates sample-specific "delta" for an input image, which is combined with this input image to generate a new image within the same category. Besides, an adversarial delta matching loss is designed to link the above two subnetworks together. Extensive experiments on five few-shot image datasets demonstrate the effectiveness of our proposed method.

==> sections/figures_tables/framework_detail.tex <==
\begin{figure}[t]
\begin{center}
\includegraphics[scale=0.38]{./figures/framework_detail.png}
\end{center}
\caption{Architecture of our reconstruction subnetwork and our generation subnetwork. In the generation subnetwork, $\tilde{\bm{x}}_2$ is generated based on the random vector $\bm{z}$ and the conditional image $\bm{x}_1$. In the reconstruction subnetwork, the target image $\bm{x}_2$ is reconstructed based on the conditional image $\bm{x}_1$ and the delta between $\bm{x}_1$ and $\bm{x}_2$. Best viewed in color}
\label{fig:framework_detail} 
\end{figure}

==> sections/figures_tables/motivation.tex <==
\begin{figure}[t]
\begin{center}
\includegraphics[scale=0.1]{./figures/motivation.jpg}
\end{center}
\caption{Illustration of our DeltaGAN. In the training stage, we extract real deltas from same-category seen image pairs. In the testing stage, given a conditional unseen image, we generate fake sample-specific deltas for this image to produce diverse and realistic unseen images}
\label{fig:motivation_illustration} 
\end{figure}

==> sections/figures_tables/network_design_supple.tex <==
\setlength{\tabcolsep}{5pt}
\begin{table}[t]

  \caption{Ablation studies of our loss terms and alternative network designs on Animal Faces dataset} 
  \centering
  %\fontsize{8}{8}\selectfont
  \begin{tabular}{lrrr}  
    \toprule[0.8pt]
     Setting& Accuracy(\%) $\uparrow$ & FID $\downarrow$  & LPIPS $\uparrow$ \cr
    \hline
    %  w/o $\mathcal{L}_{1}$ & 58.68 & 100.21   &  0.4191   \cr
    
    %  w/o $\mathcal{L}_{ms}$ & 50.08 &121.74   &  0.2976  \cr
    
    %  w/o $\mathcal{L}_{fm}$ & 59.17 & 95.82   & 0.4324     \cr
     
    %  w/o $\mathcal{L}_{c}$ & 42.21 &  196.18  &  0.4119    \cr
     
    %  w/o $\mathcal{L}^I_{adv}$ & 52.18  &  139.46  &  0.3912    \cr
    % % Simple $D_1$ & 57.12 &115.11  & 0.4553       \cr
    % \hline
     w/o $\mathcal{L}_{1}$ & 58.68 & 100.21   &  0.4191   \cr
    
     w/o $\mathcal{L}_{ms}$ & 50.08 &121.74   &  0.2976  \cr
    
     w/o $\mathcal{L}_{fm}$ & 59.17 & 95.82   & 0.4324     \cr
     
     w/o $\mathcal{L}_{c}$ & 42.21 &  196.18  &  0.4119    \cr
     
     w/o $\mathcal{L}^I_{adv}$ & 52.18  &  139.46  &  0.3912    \cr

    Simple $D_1$ & 54.53 & 129.17 & 0.3012       \cr
    
    Simple $D_2$ & 58.01 & 109.54 & 0.4401        \cr
    
    Simple $D_3$ & 59.51 & 94.12 &  0.4392       \cr
    
    % simple $D_4$ &  & 104.56 & 0.4753       \cr
    \hline
    Linear delta & 53.89 & 122.71 & 0.4091 \cr
    \hline
    DeltaGAN & $\textbf{60.31}$ &$\textbf{89.81}$  & $\textbf{0.4418}$  \cr
    \bottomrule[0.8pt]
  \end{tabular}
%   \vspace{0.1mm}
  \label{tab:network_design_supple}
\end{table}

==> sections/figures_tables/two_dataset_combination.tex <==
\begin{figure*}
\begin{center}
\includegraphics[scale=0.16]{./figures/limitation_two_datasets.png}
\end{center}
\caption{Images generated by F2GAN, FUNIT, and our DeltaGAN in 3-shot setting on a combination of Flowers and Animal Faces datasets. The conditional images are in the left three column.} 
\label{fig:combination_datasets} 
\end{figure*}

==> sections/figures_tables/visualization_comparison_supple.tex <==
\begin{figure*}[t]
\begin{center}
\includegraphics[scale=0.33]{./figures/comparison_supple.jpg}
\end{center}
\caption{Images generated by DAGAN, F2GAN, and our DeltaGAN in $3$-shot setting on two datasets (from top to bottom: Animal Faces and NABirds). The conditional images are in the left three columns}
\label{fig:visualization_compare_supple} 
\end{figure*}


==> sections/includes.tex <==
\usepackage[utf8]{inputenc} % allow utf-8 input
%\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography

\usepackage{algorithm,algpseudocode}
\usepackage{amsmath}
\usepackage{amsfonts}
% \usepackage{amssymb}
\usepackage{subcaption}
\usepackage{bm}
%\usepackage{tikz}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}

\usepackage{graphicx}
\usepackage[american]{babel}
\usepackage{hyperref}
\usepackage{caption}
\usepackage{multirow}
\usepackage{enumitem}
\def\A{{\bf A}}
\def\a{{\bf a}}
\def\B{{\bf B}}
\def\b{{\bf b}}
\def\C{{\bf C}}
\def\D{{\bf D}}
\def\d{{\bf d}}
\def\E{{\bf E}}
\def\e{{\bf e}}
\def\F{{\bf F}}
\def\f{{\bf f}}
\def\G{{\bf G}}
\def\g{{\bf g}}
\def\k{{\bf k}}
\def\K{{\bf K}}
\def\H{{\bf H}}
\def\h{{\bf h}}
\def\I{{\bf I}}
\def\L{{\bf L}}
\def\M{{\bf M}}
\def\m{{\bf m}}
\def\n{{\bf n}}
\def\N{{\bf N}}
\def\BP{{\bf P}}
\def\R{{\bf R}}
\def\BS{{\bf S}}
\def\s{{\bf s}}
\def\t{{\bf t}}
\def\T{{\bf T}}
\def\U{{\bf U}}
\def\u{{\bf u}}
\def\W{{\bf W}}
\def\w{{\bf w}}
\def\X{{\bf X}}
\def\Y{{\bf Y}}
\def\Q{{\bf Q}}
\def\x{{\bf x}}
\def\y{{\bf y}}
\def\Z{{\bf Z}}
\def\z{{\bf z}}
\def\0{{\bf 0}}
\def\1{{\bf 1}}
\def\SS{{\bf S}}
\def\ME{{\mathbb E}}
\def\MF{{\mathcal F}}
\def\MG{{\mathcal G}}
\def\MI{{\mathcal I}}
\def\ML{{\mathcal L}}
\def\MN{{\mathcal N}}
\def\MO{{\mathcal O}}
\def\MT{{\mathcal T}}
\def\MX{{\mathcal X}}
\def\SW{{\mathcal {SW}}}
\def\MW{{\mathcal W}}
\def\MY{{\mathcal Y}}
\def\BR{{\mathbb R}}
\def\MS{{\mathcal S}}
\def\MC{{\mathcal C}}
\def\ph{\mbox{\boldmath$\phi$\unboldmath}}
\def\vp{\mbox{\boldmath$\varphi$\unboldmath}}
\def\pii{\mbox{\boldmath$\pi$\unboldmath}}
\def\Ph{\mbox{\boldmath$\Phi$\unboldmath}}
\def\pss{\mbox{\boldmath$\psi$\unboldmath}}
\def\Ps{\mbox{\boldmath$\Psi$\unboldmath}}
\def\muu{\mbox{\boldmath$\mu$\unboldmath}}
\def\Si{\mbox{\boldmath$\Sigma$\unboldmath}}
\def\lam{\mbox{\boldmath$\lambda$\unboldmath}}
\def\Lam{\mbox{\boldmath$\Lambda$\unboldmath}}
\def\Gam{\mbox{\boldmath$\Gamma$\unboldmath}}
\def\Oma{\mbox{\boldmath$\Omega$\unboldmath}}
\def\De{\mbox{\boldmath$\Delta$\unboldmath}}
\def\de{\mbox{\boldmath$\delta$\unboldmath}}
\def\Tha{\mbox{\boldmath$\Theta$\unboldmath}}
\def\tha{\mbox{\boldmath$\theta$\unboldmath}}
\def\etal{{\em et al.\/}\,}
\def\eg{{\em e.g.\/}\,}
\def\tr{\mathrm{tr}}
\def\exp{\mathrm{exp}}
\def\rank{\mathrm{rank}}
\def\diag{\mathrm{diag}}
\def\dg{\mathrm{dg}}
\def\argmax{\mathop{\rm argmax}}
\def\argmin{\mathop{\rm argmin}}
\def\vecd{\mathrm{vec}}
\def\ie{\textit{i.e.}, }
\def\gradi{{\nabla \mathbf \I}}
\newcommand{\row}[2] {#1_{#2 \cdot}}
\newcommand{\col}[2] {#1_{\cdot #2}}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}

==> sections/rebuttal.tex <==
We thank all the reviewers for recognizing our novelty and contribution.

\noindent\textbf{To Reviewer#1\&#2:}

\noindent\textit{Q: Difference between training classes and testing classes.}

\noindent\textit{A:}




\noindent\textbf{To Reviewer#1\&#4:}

\noindent\textit{Q: Optimization items and hyper-parameter tuning.}

\noindent\textit{A:} Compared with baselines such as MatchingGAN, F2GAN, and other generative papers such as StarGAN, the number of our DeltaGAN loss terms are acceptable. In Equation (11), the first four loss items related discriminators can be merged as one GAN loss. Besides, most of those losses are centered around the proposed deltas, which is designed to force network to learn meaningful sample-specific deltas.

\noindent\textit{Q: Gains from architecture and cherry-picking of the results.}

\noindent\textit{A:} In fact, our model architecture is similar to MatchingGAN and F2GAN (see Table 4. in Supplementary), our model has even fewer parameters than MatchingGAN and F2GAN. To obtain convincing experimental results, we conduct extensive experiments on five datasets including evaluation metrics such as LPIPS and FID in Table 1 , and also report the results of downstream tasks such as few-shot image classification in Table 2 and low-shot image classification in Table 8 in supplementary.



\noindent\textbf{To Reviewer#2:}

\noindent\textit{Q: Identity preserving.}

\noindent\textit{A:} Our method is designed to learn intra-category deltas to generate diverse images, therefore the images generated from our DeltaGAN belong to the category of the input image,  and we don't put restriction on the identity preserving. To demonstrate the generated images are category-preserving, we use generated images to augment few-shot image classification in Table 2 in the main paper and low-shot classification in Table 8 in supplementary.


\noindent\textbf{To Reviewer#3:}

\noindent\textit{Q: Writting improvement.}

\noindent\textit{A:} The dimension of generated images is 96 $\times$ 96, which is same as the dimension of the input images, and we report it in Table 1 in supplementary. Thanks for your suggestions about the writting improvement for section 3, and we will improve it in later version. The triplet should be written as $\{\mathrm{\hat{D}}_{I}(\bm{x}_1), \mathrm{\hat{D}}_{I}(\bm{x}_2), \bm{\Delta}_{x_1}^{r}\}$ in anywhere, and we will correct it in the later version.



\noindent\textbf{To Reviewer#4:}

\noindent\textit{Q: Illustration of the property of capturing delta from same-category pairs.}

\noindent\textit{A:} As is shown in Figure 3, in the reconstruction subnetwork, the difference between $E_{\delta}(\bm{x}_1)$ and $E_{\delta}(\bm{x}_2)$ is fed into encoder $E_r$ to reconstruct $\bm{x}_2$, we assume that $E_{\delta}(\bm{x}_1)$ is same valid as $E_{\delta}(\bm{x}_2)$ and the information of $E_{\delta}(\bm{x}_1)$ is not ignored, $E_r$ take the difference as input to reconstruct $\bm{x}_2$, thus, the mentioned shortcut doesn't exist because of the existence of the real delta extracted from $E_{\delta}(\bm{x}_1)$ and $E_{\delta}(\bm{x}_2)$. Besides, we report result of without real delta referred to ``w/o real delta" in Table 3 in the main paper. In detail, we cut off the links between real delta and fake delta by removing the reconstruction subnetwork and adversarial delta matching loss (\emph{i.e.}, removing $\{\mathcal{L}^M_{D},\mathcal{L}^M_{GD}, \mathcal{L}_{1}, \mathcal{L}_{fm}\}$) . Compared with DeltaGAN, both diversity and realism are significantly degraded, we think that generation subnetwork fails to generate meaningful deltas without the guidance of real delta extracted from reconstruction subnetwork. We also exchange sample-specific deltas within same categories referred as ``SC delta" in Table 3 and exchange sample-specific deltas across different categories referred as ``DC delta" in Table 3, the corresponding performance are degraded compared with our DeltaGAN, which demonstrate the effectiveness and importance of the design of sample-specific deltas.

% \noindent\textit{Q: How real delta works.}

% \noindent\textit{A:}

\noindent\textit{Q: The role of mode seeking loss.}

\noindent\textit{A:} We conduct ablation study ``w/o real delta" in Table 3, in which the guidance of real delta is removed, solely using mode seeking loss cannot generate meaningful deltas, with both diversity and realism significantly downgraded. Besides, mode seeking loss is not suitable to be added in FUNIT due to it doesn't support stochastic sampling.  



\noindent\textit{Q: Diversity difference between our method and FUNIT.}

\noindent\textit{A:}  We have summarized the diversity differences between our DeltaGAN and FUNIT. Our DeltaGAN consists of category-relevant diversity (\emph{resp.}, object appearance) and category-irrelevant diversity (\emph{resp.}, object pose), we can see the third-to-last row in Figure 4, the generated images are category-preserving with rich pose diversity and appearance diversity. FUNIT is designed to disentangle a image into category-relevant code and category-irrelevant code. In this way, combining different category-irrelevant codes (\emph{resp.}, object poses) with the input of category-relevant code (\emph{resp.}, object appearance) only introduce category-irrelevant diversity. As is shown in Figure 9 of FUNIT,  the generated images show appearance variance due to the failure of disentanglement. 

\noindent\textit{Q: Meaning of category relevant/irrelevant features.}

\noindent\textit{A:} Our DeltaGAN is designed to learn sample-specific delta, which is related to the input sample and consists of both category-relevant feature and category-irrelevant feature. As is shown in Figure 4 in main paper, the generated images in the third-to-last row show rich category-relevant diversity (\emph{resp.}, diverse appearances) and category-irrelevant diversity ((\emph{resp.}, diverse poses). Due to the learned deltas are sample-specific, the generation subnetwork can combine random vector $\bm{z}$ with the input image $\bm{x}_1$ to form reasonable sample-specific delta, which is used to generate reasonable image.



\noindent\textit{Q: Detailing where FUNIT fails compared with our DeltaGAN.}

\noindent\textit{A:} The experimental setting of our DeltaGAN is different from the setting of FUNIT. FUNIT need to take use of training content images to generated diverse images based on the provided class image, and the number of the generated images is limited. While our DeltaGAN only take given test images to generate diverse sample-specific deltas and generate diverse images. Compared with FUNIT, the generated images by our DeltaGAN can introduce category-relevant diversity and category-irrelevant diversity, while the generated images from FUNIT only with category-irrelevant diversity by changing the category-irrelevant codes.


\noindent\textit{Q: N-shot setting, Visual comparison results and FID calculation.}

\noindent\textit{A:} In N-shot setting, delta is also conditioned on single image. Conducting N-shot setting by repeating N-times 1-shot experiment. In Figure5, DAGAN task one conditional image as input to generate new image, we arrange generated images in order to the conditional images. The images generated by F2GAN are similar to conditional images due to weak fusion ability, thus we visualize the generated images similar to the conditional image according to the order of conditional images. As for FID calculation, DRIT++ using 1000 images to calculate FID, COCO-FUNIT takes hundreds of images as input to calculate FID.

==> sections/response.tex <==
\noindent\textbf{}Dear Editor-in-Chief, Associate Editor, and Reviewers,
\\

\noindent\textbf{}We would like to thank the Associate Editor and the reviewers for their elaborative comments and constructive suggestions. We have carefully addressed the
comments of each reviewer by adding more discussions and experiments, with
the manuscript revised accordingly. The detailed responses are on the following
pages. In this response file, we use {red} color to mark the tables and figures from
the manuscript, with their indices based on the revised manuscript. To clearly
show the revisions in the manuscript, we highlight the modified parts with red
color, which are uploaded as the supplementary file (diff.pdf).
\\

\noindent\textbf{}Sincerely,

\noindent\textbf{}Yan Hong,  Li Niu, Jianfu Zhang, Liqing Zhang



 \clearpage
 
 %\maketitle
\thispagestyle{empty}
%We thank all the reviewers for recognizing our novelty and contribution.

\noindent \textbf{To Reviewer1}

\noindent\textbf{Question 1:} 
\noindent\textbf{Answer 1:}: 
